Conformer-Based Self-Supervised Learning for Non-Speech Audio Tasks

Representation learning from unlabeled data has been of major interest in artificial intelligence research. While self-supervised speech representation learning has been popular in the speech research community, very few works have comprehensively analyzed audio representation learning for non-speech audio tasks. In this paper, we propose a self-supervised audio representation learning method and apply it to a variety of downstream non-speech audio tasks. We combine the well-known wav2vec 2.0 framework, which has shown success in self-supervised learning for speech tasks, with parameter-efficient conformer architectures. Our self-supervised pre-training can reduce the need for labeled data by two-thirds. On the AudioSet benchmark, we achieve a mean average precision (mAP) score of 0.415, which is a new state-of-the-art on this dataset through audio-only self-supervised learning. Our fine-tuned conformers also surpass or match the performance of previous systems pre-trained in a supervised way on several downstream tasks. We further discuss the important design considerations for both pre-training and fine-tuning.

==> discussion.tex <==
Please write your thoughts and comments here.

Yun

1. We state one of our contributions as "closing the gap between self-supervised and supervised pre-training".
But most of the supervised pre-training baselines (those in the transfer learning paper) only used feature-based learning, while we applied fine-tuning.
Is this a fair comparison? How should we qualify our conclusion?

Sangeeta: I had brought up this concern in one of our meetings (with You, me and Anurag). And Anurag had suggested to be blind to how one is using pre-trained metwork. IMO, there is no other way of putting this as a conclusion. If we don't want to say this, we will have to remove this contribution. What does Anurag have to say to this?

Yun: Let's discuss with Anurag in Messenger. I feel that our current claim may be challenged by reviewers. Maybe we can just admit that it's not a fair comparison, but the transfer learning paper is the only baseline available.

Sangeeta: I agree with you on "I feel that our current claim may be challenged by reviewers".

2. When I was writing a "layman's abstract" for the SRT review,
I realized we weren't emphasizing enough in our paper that our self-supervised pre-training is most helpful for scenarios with limited labeled data.
We should emphasize this in the abstract, introduction, and conclusion. What do you think?

Sangeeta: Umm, I am not really sure of this claim. If you look at Kinetics and DCASE, it's not that the improvement (S vs. SS) is more in DCASE as compared to Kinetics. Can you talk more about what makes you say "most helpful for scenarios with limited labeled data"? If you just have AudioSet in mind for this claim, I will not really write it because then one tries to find similar trend in Table 3 which doesn't exist. What do you think?

Yun: I'm saying our work is "most helpful for scenarios with limited labeled data" because Fig. 2 show that the improvement occurs mostly for Balanced AudioSet. But yes, in Table 3, the improvement compared with the baselines isn't well correlated with the amount of labeled data.
Shall we just say "Our work can be useful for scenarios with limited labeled data", avoiding comparative terms like "most" or "especially"? I'd like to emphasize the practical use of our work.

Sangeeta: Using such a generic way of stating it's usefulness in case of limited data is not helpful IMO. If there is no comparative stmt, then how is our work different from any other SS's use-case? SS is meant to work for data with less data. In short, I am still not convinced in bringing out the "limited data" point as a different category if there are no strong stmts to be made.
